SABER-6D: Shape Representation Based Implicit Object Pose Estimation

In this paper, we propose a novel encoder-decoder architecture, named SABER, to learn the 6D pose of the object in the embedding space by learning shape representation at a given pose. This model enables us to learn pose by performing shape representation at a target pose from RGB image input. We perform shape representation as an auxiliary task which helps us in learning rotations space for an object based on 2D images. An image encoder predicts the rotation in the embedding space and the DeepSDF based decoder learns to represent the object's shape at the given pose. As our approach is shape based, the pipeline is suitable for any type of object irrespective of the symmetry. Moreover, we need only a CAD model of the objects to train SABER. Our pipeline is synthetic data based and can also handle symmetric objects without symmetry labels and, thus, no additional labeled training data is needed. The experimental evaluation shows that our method achieves close to benchmark results for both symmetric objects and asymmetric objects on Occlusion-LineMOD, and T-LESS datasets.

==> sec/6_Limitations.tex <==
\section{Limitations and Future Work}
Our approach doesn't explicitly utilize the texture cues from the image or the CAD model. Instead, it utilizes the features from SurfEmb which depend on both texture and geometry simultaneously. Employing another expert that models the texture cues explicitly will enable us to model distribution which would help us handle objects like SphereX on Symsol-II where the shape expert cannot contribute towards the distribution.     

==> sec/7_rebuttal.tex <==
\begin{table}[h]
\centering
	\begin{tabular}{l|c|c|c}
		 % \textbf{Method} & \textbf{GDRN} & \textbf{ SurfEmb} & \textbf{CosyPose} &\textbf{SC6D}&\textbf{Ours}\\ \hline
		 % \textbf{Method} & \textbf{GDRN} & \textbf{ SurfEmb} & \textbf{CosyPose} &\textbf{SC6D}&\textbf{Ours}\\ \hline

           \textbf{Method} & \textbf{SC6D} & \textbf{Ours} & \textbf{Ours-DH} \\\hline
            \textbf{Sym} & \xmark & \xmark & \cmark  \\\hline
           
           % \textbf{Stage} & \textbf{1} & \textbf{1} & \textbf{1} &\textbf{2}\\
           
% 		 \hline
% 		 Ape		& 80.2 &53.3 & 81.4&69.97\\
% 		 Can		& 90.1 &86.5 & 94.7&83.08\\
% 		 Cat		& 61.2 &73.4 & 55.2&56.66\\
% 		 Driller	& 94.8 &92.8 & 86.0&86.31\\
% 		 Duck		& 77.6 &62.8 & 79.7&64.53\\
% 		 Egg box	& 72.9 &95.3 &65.6 &87.64\\
% 		 Glue		& 77.5 &92.5 &52.1 &78.71\\
% 		 Puncher	& 92.9 &76.7 &95.5 &89.16\\
		 \hline
		 \hline
		 AR     &0.79 &0.76 &0.76 \\
	\end{tabular}
	\caption{Results on 11 T-LESS Continuous Symmetric objects. Ours-DH refers to our correspondence regression approach trained by removing symmetry ambiguities during data handling instead of handling during training using our loss. Sym refers to using symmetry prior.}	
	\label{table:csym}
% 			\vspace{-1.0em}
\end{table}


==> sec/unused.tex <==
We employ uncertainty estimation by utilizing a mask prediction network and estimating the pose. Instead of estimating visible masks, we predict full object masks even for occluded objects. The mask and pose both are estimated from the network. By comparing the two entities, mask, and pose, we can estimate how uncertain we are about the estimated pose. We render the object using the estimated pose and compare that with the estimated mask to compute a score based on their alignment. Intuitively, if the masks align well, it means that the network is very confident in both the predictions and the network is confident. Besides, our approach can also be used to speed up the inference process of SurfEmb. SurfEmb needs to follow a rigorous inference process as the same 2D feature is matched to multiple valid 3D points for symmetric objects which makes it difficult to apply PnP to estimate 3D pose. Instead, the feature image/correspondences from SurfEmb can be employed as input to our pipeline to predict pose estimates much faster.

In conditional symmetric objects like a coffee mug with a handle that becomes symmetric when the handle is masked, our approach based on correspondences can handle occlusions better as we can compute a score for each rotation by comparing corresponding features at different orientations. IPDF needs to have

Uncertainty estimation helps us understand how reliable the estimated modes are.

In addition, we also propose a mechanism to estimate object pose uncertainty based on occlusions which enables us to understand when to trust the estimated pose. Our approach is agnostic to a network architecture and can be extended to any other strong encoders. 

Besides pose distribution, uncertainty estimation of a pose is crucial and gives an insight into whether to trust the pose estimate or not

\subsection{Uncertainty Based on Occlusions}
We use the estimated mask and the estimated pose to get an uncertainty metric employing intersection over union metric. We predict full object masks even for occluded objects. We render the object CAD model with the estimated pose to generate a projected mask. We compare the estimated mask and the projected mask and compute the IoU score for the estimated pose. When the masks align perfectly, it indicates that the mask and the pose estimates from the network are confident. For example, in the cases of heavy occlusions, the predicted mask and projected mask don't align perfectly, and comparing masks serves as a good metric to indicate the confidence of the pose estimate. As shown in Figure 

\begin{table}[!htp]\centering
\caption{Ablations with positional encoding and sampling strategy for training. Rotation encoding refers to the rotation encoding employed in the approach. IPDF refers to positional encoding proposed in IPDF where positional encoding from NeRF is applied  to rotation matrix elements separately. Wigner matrices refer to representing rotation matrices as wigner-D matrices. Cube PE refers to our positional encoding where NeRF based positional encoding is applied on 8 vertices of Cube with rotation applied to vertices. Sampling refers to the rotations sampled for each image in a batch. Random refers to random sampling from uniform distribution. Grid refers to sampling from the distribution estimated using ground truth pose and features. The number indicates the level of recursion in the healpix grid. The approach gets more accurate when we sample from finer grid. Scores refers to scores employed to estimate the final distribution. S refers to SDF based score and F refers to feature based score. The combined result of SDF and Feat scores provides the best accuracy. \tolga{which dataset? why is IPDF so close to ours now while in others it's really bad?} \shishir{It was ours with IPDF PE, not IPDF approach.}\ben{make sure to associate this with expert models from method section ablating them}} 
\label{tab: }
%\scriptsize
% \setlength{\tabcolsep}{8pt}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{l|ccccccccc}
% \toprule
Encoding &IPDF PE &Wigner &Cube PE &Cube PE &Cube PE &Cube PE &Cube PE \\\hline
Sampling &grid 6 &grid 6 &random &grid 6 &grid 7 &grid 7 &grid 7 \\\hline
Scores &F+S &F+S &F+S &F+S &S &F &F+S \\\hline
LL &10.09 &8.59 &? &10.2 &10.17 &10.02 &10.5 \\
% \bottomrule
\end{tabular}
\end{table}


For the uncertainty estimation network, we use the evaluation dataset provided in the T-Less dataset with heavy occlusions and different scenes. We demonstrate the performance of our uncertainty estimation using plots similar to Deep Bingham where the uncertain samples are removed with an increasing confidence threshold and the accuracy is computed with the remaining samples. If the accuracy is proportional to the threshold value, it indicates that the threshold is valid.  Our results are presented in Figures. 

 Besides, we also propose an uncertainty confidence metric based on comparing pose and mask predictions from the network which serves as a confidence metric for further actions. Our approach can also be extended to improve the inference speed of SurfEmb without compromising accuracy. Our framework can handle asymmetric and symmetric objects indifferently during pose distribution estimation and uncertainty estimation.

 \shishir{a sbrief description of tables Starts here. Will be removed}{Summary of each Table and results}
Table 1. In Symsol-I, we perform better than NF which is best performing approach. WE are better in both low data regime, full data and less iterations. NF is prone to overfitting in some objects(icosa and cylinder)with less data which is evident from decreasing results from 100k to 900k iterations. All groundtruth symmetry labels are provided and hence it is more challenging than others.

\paragraph{Table 2}: We suffer mostly in icosa object. NF also suffers in the case of training with 100k iterations. Other objects are closeby. Spread = angular error * probability of that mode iterated over all the modes.
\paragraph{Table3}:We are behind in Symsol2 compared to NF. We are better than them in low-data regime. In low data and full data, the sphere seems to suffer more compared to other objects. This is because there is no geometry aspect to rely on in case of sphere and need to completely rely on Surfemb features. Tet is still not done. could improve a bit more. I should add spyropose also with 10k results. we are better than them also. Only 1 ground truth rotation is provided for evaluation unlike symsol-I where all the groundutrh samples are provided


\paragraph{Table 4}: Only one ground truth label is provided for evaluation. We ar behind sypropose. the result in the table is with surfemb features from  pbr data. Currently, an experiment is running with pbr+real features. Hope that improves the result. The datset doesnlt contain inplane rotations. Otehr networks have to interpolate between existing dataset rotations where are we try to learn rotations in complete space. There are also many minute symmetry breaking features in T-Less objects. Reasons in case of less accuracy:The slight loss in accuracy could be the result of SurfEmb features which are trained on images with blur included in the augmentations which can sometimes suppress the minute features. Since spyropose is a contrastive learning approach, it focuses more on distinguishing portions in the image. In our approach, we use shape and features

\paragraph{Table5}: Ablations: Our positional encoding works better than wigner and ipdf's positional encoding. Our Sampling is better than random(tbd) and it improves when we save distributions on grid 7 healpix and sample from that to sample more near modes. The finer the better so that we stay close to the actual groundtruth distribution. Combining both Shape and SurfEmb features is justified by improved performance when both are combined. 

We employ an architecture similar to IPDF with a ResNet50 image encoder and an MLP each for inferring unnormalized SDF and SE measures. The image encoder encodes the image as a global latent vector which is concatenated with the positional encoded rotation matrix and passed through two MLPs to get unnormalized SDF and SE measures. For a given image, we sample $K$ rotations, to learn the distribution at $K$ discrete points in $SO(3)$ space. To train the network, for a given image, we generate the supervision signal using pre-trained SDF and SE MLPS. For a given image, $\Img$, and a ground truth rotation, $\Rot_\mathrm{gt}$, the image aligned point cloud, $\X$, is transformed using $\Rot_\mathrm{gt}$ and passed through SE MLP to get canonical per-point features. Then, for a given rotation, $\Rot$, we transform the image aligned point cloud, $\X$, with $\Rot$ and pass through the SurfEmb MLP to get per-point features for that specific rotation. We estimate the $L_2$-norm between per-point features corresponding to ground truth rotation and current rotation, $\Rot$ which is treated as the SE score for that rotation matrix for a given image. The intuition is that the point cloud can be transformed to any symmetric configuration and the per-point features are still preserved and hence will have a low score for symmetric configurations. On the other hand, the rotations that don't align the point cloud with any of the symmetric configurations will get higher scores. 
Similarly, we pass the transformed point cloud rotated using a rotation, $\Rot$, through SDF network and estimate the $L_0$-norm which is treated as SDF score for that rotation. For a given image, this procedure is repeated for all the $K$ rotations to gather scores for all the rotations which are used to supervise the network by estimating the GKL between the generated scores and inferred scores.                   

IPDF refers to positional encoding proposed in IPDF where the positional encoding from NeRF\cite{mildenhall2020nerf} is applied to rotation matrix elements separately. Wigner matrices refer to representing rotation matrices as wigner-D matrices with level 5 encoding. Cube PE refers to our positional encoding where NeRF based positional encoding is applied on 8 vertices of Cube with rotation applied to vertices.

\section{Additional Results on T-Less}
On T-Less, we report results for normalizing flow by retraining their approach with T-Less data as they don't provide results for T-Less dataset in their paper. We observe that Normalizing flow performs marginally better compared to our approach with the same number of iterations and performs much better compared to our approach with 200k iterations. We believe the result is because the T-Less dataset doesn't contain in-plane rotations as we only consider real training data without any occlusions. Since, there are no in-plane rotations, the learning subspace of rotations reduces by a large amount for other approaches like Normalizing flow, Spyropose and IPDF. On the other hand, we try to learn the distribution over the entire SO3 without assuming that learning should only be focused on a subspace of rotations. This carries an implicit advantage to approaches that only learns from image training data without considering information from a CAD model. This is similar to pose estimation for upright objects in the Linemod dataset where training with images containing only upright poses focuses the learning problem on only a subspace of rotations. 

==> sec/unused_tolga.tex <==

\tolga{I did not revise after this point.}.\\
\begin{comment}
Below is a proof sketch:
\begin{proof}
We will consider the vectorized versions of our variables $\rb:=\vec{\Rot}$ and $\x^\prime:=\vec{\X^\prime}$ and assume $p(\rb\given{\Img})=p(\Rot\given{\Img})$ and $p(\x^\prime\given{\Img})=p(\X^\prime\given{\Img})$. Let $\C=\Pi(\Rot_\mathrm{gt}^{\top}\X_0)$ denote the visible part of the model, assumed to be a constant. Then, the two distributions can be related by the \emph{change of variables}:
    \begin{align}
        p(\rb\given{\Img})= p(\x^\prime \given{\Img}) \cdot |\J|,
   \end{align}
   where
   \begin{align}
   \J := \frac{\diff \x^\prime}{\diff \rb}=\frac{\diff \vec{\Rot\C}}{\diff\rb} = \frac{\diff \left(\left(\C^\top \otimes \Id_{N_X}\right)\rb\right)}{\diff\rb}=\C^\top \otimes \Id_{N_X}.
   \end{align}
    Hence the determinant of the Jacobian, $|\J|:=|\det\J|$, is independent of $\Rot$:
    \begin{align}
    |\J|=|\C^\top \otimes\Id_{N_X}|=\sqrt{|(\C^\top \otimes\Id_{N_X})^\top(\C^\top \otimes\Id_{N_X}))|}=\sqrt{|\C\C^\top|}.
    \end{align}
    As the canonical model $\X_0$ and $\Rot_{\mathrm{gt}}$ are known, $|\J|$ remains constant leading to: 
    \begin{align}
    p(\Rot\given{\Img})= p(\X^\prime \given{\Img}) \cdot \sqrt{|\C\C^\top|}\propto p(\X^\prime \given{\Img}).\nonumber\tag*{\qedhere} %\qedhere\popQED
    \end{align}
    %\qed
\end{proof}
\end{comment}

\begin{wrapfigure}[12]{r}{.4\linewidth}
\vspace{-8mm}
    \centering
    \includegraphics[width=\linewidth]{images/distequiv.pdf}
    \vspace{-6mm}
    \caption{\normalfont Training by ensuring distributional invariance \ben{To be reworked and made consistent with text}.}
    \label{fig:distequiv}
\end{wrapfigure}
Due to these drawbacks, we take a different path and assume the availability of a CAD model $\X=\{\x_i\in\R^3\}\in\R^{N_X\times 3}$ during training. We propose a new way to compute $p(\Rot\given{\X})$, the CAD-conditional probability density over $SO(3)$, explicitly. We do so by leveraging the recent SurfEmb~\cite{haugaard2022surfemb}, which models continuous 2D-3D correspondence distributions $p(\x,\pt\given{\Img})=p(\pt\given{\Img})p(\x\given{\Img,\pt})$ over the surface of objects, where $p(\pt,\given{\Img})$ denotes the discrete distribution over image coordinates. SurfEmb consists of a network supervised to maximize the probability of the ground truth coordinates.  
To be continued...
\begin{comment}
\begin{align}
    p(\Rot\given{\Img}) &=\int p(\Rot\given{\X,\Img}) p (\X\given{\Img}) \diff\X = \int p(\Rot\X\given{\Img}) p (\X\given{\Img}) \diff\X= p(\X^\prime \given{\Img}).
\end{align}
    
\begin{align}
    p(\Rot\given{\Img}) &=\int p(\Rot\given{\X,\Img}) p (\X\given{\Img}) d\X\\
    &\approx p_\mathrm{SDF}(\Rot\given{\X,\Img})p_\mathrm{SE}(\Rot\given{\X,\Img})\\
    &\propto \exp\left(-\|\mathrm{SDF}(\Rot\X)\|_0 - \|G_{\theta}(\Rot\X)-G_{\theta}(\Rot_0\X)\|_2\right),
\end{align}
where $\X$ is the ground truth model (corresponding to $\X^\prime$ in Eq. 8). $\Rot_0$ is the GT rotation bringing the 3D model to the image frame.
\end{comment}
Since we wok with unnormalized densities, to learn the parameters $\params$ of $f_{\params}$, we leverage a generalized version of KL-divergence that can work with unbalanced distributions~\cite{miller2023simulation} by aligning ${\mur}$ to ${\muc}$:
\begin{align}
    \label{eq:GKL}
    \mathrm{GKL}\infdivx{\mur}{\muc}  = \sum\limits_{i=1}^n \left(-\log\left(\frac{a^{\muc}_i}{a^{\mur}_i}\right) + \left(\frac{a^{\muc}_i}{a^{\mur}_i}\right) -1\right){a^{\mur}_i},
\end{align}
where $\ab=\{a^{\mur}_i\}$ and $\{x^{\mur}_i\}, i=1,\ldots, m$ denote the weights and locations of a discrete measure $\mur = \sum\nolimits_{i=1}^m a_i \delta_{x_i}, a_i\geq 0$, where $\delta_{x}$ is a Dirac delta at $x$.

\vspace{2mm}\noindent\textbf{Loss and Details}
For a given image, $\Img$, with ground truth rotation, $\Rot_{g}$, our goal is to learn the probability distribution of rotations. IPDF tries to learn the distribution by maximizing the probability of ground truth rotation and minimizing the probability of randomly sampled rotations. In our approach, we assume that the CAD model, $\X$, of the object is available to us. We initially employ SurfEmb to learn surface features on the CAD model, $\Z$, using synthetic data rendered from the CAD model. Prior approaches don't assume that a CAD model is available and they focus on maximizing the probability of one single rotation label provided during training. In our approach, we use the single rotation label and the features from SurfEmb to convert the problem of learning pose distribution into a completely supervised pipeline by formulating loss between pose distributions instead of relying on maximizing a single point estimate. Specifically, we employ per-point surface features, $\Z$, on the CAD model surface, $\X$, and the ground truth rotation, $\Rot_{g}$, and the given input Image,$\Img$ to estimate score/probability for any random rotation, $\Rot_{i}$. This enables us to estimate the scores for any rotation for a given Image. So, we can supervise our network by focusing on any set of training rotations instead of focusing on a point estimate. In IPDF, every image is paired with a groundtruth rotation and $k$ randomly sampled rotations which are all equally treated as negatives. In our approach, since we know the scores for $k$ random rotations in addition to the ground truth rotation, all the rotations can contribute towards learning distribution in a meaningful manner. Besides, IPDF relies on the exhaustive sampling of images to learn the distribution effectively. On the other hand, our approach distills the knowledge from the CAD model about symmetries into the network. In the case of symmetric objects, the network doesn't have to see a similar-looking image with multiple rotation labels to learn about the symmetries. The knowledge about symmetries is encoded in the features and hence can learn about all the symmetric configurations by looking at a single image with our generated score labels. We generate two sets of scores where we measure deviation of a rotation from the given image. We generate scores using SurfEmb features which help in incorporating texture and symmetry related information. We also formulate another score purely based on object's shape where we measure the deviation between the object's shape at ground truth rotation and the object's shape and the sampled rotation.   

We employ a neural network, $D_{\theta}$, similar to IPDF, comprising a CNN encoder to encode an image, $\Img$, to a global feature vector. The global feature vector is concatenated with a rotation matrix, $\Rot_{i}$ and passed through two MLP heads to predict Feature deviation score, $o_{i}$, and Shape deviation score, $m_{i}$. The network is defined as follows,
\begin{equation}
    o_{i}, m_{i}= D_{\theta}(\Img, \Rot_{i})
\end{equation}

We generate the shape deviation score and feature deviation score for a randomly sampled rotation, $\Rot_{i}$ for a given image using the CAD model and SurfEmb Features which are used to supervise scores predicted from our network. The score estimation is described in the following section. 

\subsection{Feature based Scoring}
 For a given image,$\Img$, along with its ground truth rotation, $\Rot_{g}$, we employ a scoring method to generate scores for different rotations which are used to supervise our network.
 % This scoring mechanism converts the learning process into a completely supervised approach where scores for all rotations are known before the training whereas the contrastive learning based approach is supposed to discover different modes for a symmetric object during training.
 % In our case, we can estimate all the modes using our scoring mechanism.
 
 For a given training image, we render NOCS coordinates using ground truth rotation, $R_{g}$, to estimate the corresponding 3D points on the CAD model. The NOCS coordinates are 3d points on the CAD model which we refer to as $\X$. SurfEmb has a feature MLP, $G_{\theta}$, which is trained to predict corresponding per-point 3D features, $\Z$. The features, $\z_{j}$, corresponding to the $j^{th}$, 3d point, $\x_{j}$, in point cloud, $\X$,  is estimated as follows:
 \begin{equation}
     \z_{j}=G_{\theta}(\x_{j})
 \end{equation}
 
We transform the 3D points on the cad model with the inverse of the ground truth rotation, $\Rot_{g}$, to obtain 3d points in image pose,$\X_{g}$. We use the rotated 3D points, $\X_{g}$, to generate score for any random rotation matrix for the given viewpoint image. To estimate the score for a rotation, $\Rot_{i}$, we rotate the 3D points in image pose, $\X_{g}$, with  $\Rot_{i}$ and pass the rotated 3D points through the feature MLP to predict corresponding 3D features. The corresponding features, $\Z^{\prime}$, are compared with canonical features, $\Z$, to estimate the score, $o_{i}$, for $\Rot_{i}$ as follows: 
 \begin{equation}
 \begin{split}
     \X_{g} &= \Rot^{-1}_{g}.\X \\
     \Z_{i} &=G_{\theta}(\Rot_{i}.\X_{g}) \\
     o^{\prime}_{i}&=\norm{\Z_{i}-\Z}
      \end{split}
 \end{equation}
The score is computed by taking the distance between the per-point features of the transformed points ,$\Z^{\prime}$, and canonical features, $\Z$. The process is repeated for the desired number of rotations and scores serve as an indicator of the probability of the rotation for that given image.  This scoring metric is valid even for symmetric, conditionally symmetric objects, and textured objects as the feature MLP learns features that respect symmetry, geometry and texture. For symmetric objects, the feature distance for 3D points when transformed to another symmetric configuration will yield a smaller score compared to invalid rotations that yield a higher score. It helps in learning pose distribution as the features We use this score as a training signal to learn pose distribution. Unlike contrastive learning where only one ground truth rotation is covered for a viewpoint, our approach helps the network to learn about all the rotations by learning with our score metric.
\subsection{Shape based Scoring}
Similar to Feature based scoring, we employ another scoring mechanism to score rotations based on the deviation in the shape space. Similar to SurfEmb MLP which is trained to learn features in canonical space, we pretrain an SDF network, $H_{\theta}$, to represent the shape in canonical orientation. After training, the network can be used to measure deviation in shape space.  To estimate the score for a rotation, $R_{i}$, We transform the 3d points in image pose, $\X_{g}$, using the rotation and pass them through the shape network to predict SDF values, $\s_{i}$. The absolute maximum among the sdf values is estimated as the shape based score, $m^{\prime}_{i}$, as follows:    

 \begin{equation}
 \begin{split}
     \s_{i} &=H_{\theta}(\Rot_{i}.\X_{g}) \\
     m^{\prime}_{i}&=\max\abs{\s_{i}}
      \end{split}
 \end{equation}

\paragraph{Training and Loss}
In the previous section, we devised a method to estimate two score values for any rotation for a given image along with the ground truth rotation and CAD model. We use these score values to supervise our network. The loss if formulated between precomputed scores, $o^{\prime}_{i}, m^{\prime}_{i}$, and predicted scores, $o_{i}, m_{i}$, from neural network as follows:
 \begin{equation}
 L= \abs{m_{i}-m^{\prime}_{i}}+\abs{o_{i}-o^{\prime}_{i}}
 \end{equation}
\tolga{Please put those all in the same equation so I don't need to trace. I need no writing or descriptions. Please only write 1 equation, I don't care how big it is.}



\begin{equation}
\begin{split}
% z^{j}&=G_{\theta}(x^{j})\\
\Z_{g} &=G_{\theta}(\X_{g}) \\
% \X^{\prime}_{g} &= \Rot^{-1}_{g}.\X_{g} \
\X_{g}^{i}&=\Rot_{i}. \Rot^{-1}_{g}.\X_{g}\\
\Z^{i}_{g} &=G_{\theta}(\X_{g}^{i})  \\
o_{g}^{i^{\prime}}&=\norm{\Z^{i}_{g}-\Z_{g}} \\
% \s^{i}_{g} &=H_{\theta}(\Rot_{i}.\Rot^{-1}_{g}.\X_{g}) \\
m_{g}^{i^{\prime}}&=\max\abs{H_{\theta}(\X_{g}^{i})} \\
% m_{g}^{i^{\prime}}&=\max\abs{\s^{i}_{g}} \\
o^{i}_{g}, m^{i}_{g} &= D_{\theta}(\Img_{g}, \Rot_{i}) \\
 L&= \sum_{i,g}\abs{m^{i}_{g}-m_{g}^{i^{\prime}}}+\abs{o^{i}_{g}-o_{g}^{i^{\prime}}}
\end{split}    
\end{equation}
Notation without index for image
\begin{equation}
\begin{split}
% z^{j}&=G_{\theta}(x^{j})\\
\Z &=G_{\theta}(\X) \\
\X^{\prime} &= \Rot^{-1}_{g}.\X \\
\Z_{i} &=G_{\theta}(\Rot_{i}.\X^{\prime})  \\
o^{\prime}_{i}&=\norm{\Z_{i}-\Z} \\
\s_{i} &=H_{\theta}(\Rot_{i}.\X^{\prime}) \\
m^{\prime}_{i}&=\max_{j}\abs{s^{j}_{i}} \\
o_{i}, m_{i} &= D_{\theta}(\Img, \Rot_{i}) \\
 L&= \sum_{i}\abs{m_{i}-m^{\prime}_{i}}+\abs{o_{i}-o^{\prime}_{i}}
\end{split}    
\end{equation}
% relate 3D features that respect symmetry to the pose



\paragraph{Inference} 

% \subsection{Network Architecture}

%\begin{figure*}[th]
%    \centering
%    \includegraphics[width=\linewidth]{images/distequiv.pdf}
%    \caption{Our method seeks an rotational invariance in the distributional sense to propagate information regarding correspondence uncertainty and ambiguity to pose uncertainty and ambiguity.}
%    \label{fig:distequiv}
%\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth,scale=1]{images/IPDF.pdf}
    \caption{Corresponding Based Rotation Scoring: The scoring comprises a pre-trained CNN and a Feature MLP from SurfEmb. For a given training image, we pass the image through CNN to get the feature image. The feature image and 3D surface features are used to estimate 3D correspondences on the CAD model for the given image. Since the correspondences are estimated on the CAD model, they lie in the same canonical space as the CAD model. The Feature MLP is SurfEmb is also trained to represent features in the same canonical space. After the 3D correspondences are estimated, we pass the 3D points through Feature MLP to get corresponding per-point Features. We apply the inverse ground truth rotation on the 3D correspondence points to get a transformed point cloud. For a specific rotation, $R_{1}$, we rotate the transformed point cloud with that rotation, $R_{1}$, and compute per-point features by passing them through Feature MLP. Then, we compute the mean distance between estimated per-point features and canonical per-point features to estimate score, $Score_{R1}$, for the specific rotation. The rotation, $R_{3}$ yields lower score compared to ,$R_{1}$ and $R_{2}$ because $R_{3}$ transforms the point cloud again to canonical space. For a continuous symmetric object, even if the transformed points fall in canonical space, but are rotated about the symmetric axis, the features are still close and will yield a lower score. This happens because the SurfEmb provides us with features that respect symmetry. For a given image, we can estimate the score for any rotation matrix in the SO3 space by following this procedure. We train our network by employing this scoring mechanism to train our network similar to IPDF.}
    \label{fig:IPDF}
\end{figure*}

{
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}

Let us stick to the following convention for a consistent and quality writing: $x \in \R$ is a scalar. Capitalization does not matter for scalars, \ie, $A \in \R$. We denote vectors by lower case bold letters $\x =(x_1 \cdots x_N)^\top \in \R^N$. So $x$ is very different from $\x$. An element of a vector is also a scalar. So it is not $\x_i$ but $x_i$. Matrices are bold and capital. A square matrix is $\X =(X_{ij})\in \R^{N\times N}$. Each column of $\X$ is a vector  $\x_i$, \eg, $\X=[\dots,\x_i,\dots]$. Transposition is done via `top': $\X^\top$ and not $\X^T$. These mean different things.
$\Id_{N\times N}$ is the identity matrix. Use $\Id$ for short. Rotations belong to the special orthogonal group $\Rot\in \SO$. Together with translations $\tb\in \R^3$, they form the 3D special Euclidean group $\SE$. Use mathrm when necessary: writing $\Loss_{\mathrm{SurfEMB}}$ is good but not $\Loss_{SurfEMB}$.}

{
Additionally, `Method' is how you quote in \LaTeX. But choose when to quote. Sometimes \emph{emphasizing} or \textit{writing in Italics} is sufficient. 

\paragraph{Use of `tilde' (\char`~)} Sometimes you'll have to use tilde in your text for spacing, and I'm not talking about the math operator $\sim$. You either choose a white space or a tilde. But never both. For example, this is prohibited: Fig.~ 5. These are good practices:  Fig.~\ref{fig:IPDF} or Fig. \ref{fig:IPDF}.

Also, do not do what I just did: Always use \textbf{cleveref}. This way, you will never have to track if you write Eq or Equation or eq and etc. Instead of Fig.~\ref{fig:IPDF}, write~\cref{fig:IPDF}.

\subsection{Comparing Unnormalized Probability Densities}
I think we will eventually need to ablate on our choice for the $\ell_1$-norm score distance. Since we interpret the scores as pre-softmax probabilities, our score-loss is a distance (divergence) on the unnormalized probability space on $SO(3)$. 

\begin{dfn}[Discrete Measure]
Let us define a discrete measure $\mur$ with weights $\ab=\{a_i\}$ and locations $\{x_i\}, i=1\dots n$ as:
\begin{align}
    \mur = \sum\nolimits_{i=1}^n a_i \delta_{x_i}, \quad a_i\geq 0 
    \label{eqn:discrete_meas}
\end{align}
where $\delta_{x}$ is a Dirac delta function at $x$. When $\sum\nolimits_{i=1}^n a_i = 1$, $\mur$ becomes a \emph{probability measure} defined on the simplex $\Sigma_d\triangleq\{\x \in \R_+^n : \x^\top\one_n=1\}$ and is called \emph{normalized}.
\end{dfn}

Based on this, we could consider the following distance measures for \textbf{two unnormalized densities with identical locations}:
\begin{dfn}[Bregman Divergences]
\label{dfn:bregman}
Bregman divergences define general notions of distances or divergences for unnormalized measurers, from which we could recover specific instances. In particular, for a differentiable and convex function $\varphi:\Omega\to\R$, the Bregman divergence between $\mur$ and $\muc$ is defined as the difference between the value of $\varphi$ at $\mur$ and the first order Taylor expansion of $\varphi$ around $\muc$ evaluated at $\mur$:
\begin{align}
    \label{eq:bregman}
    \Delta_{\varphi}(\ab^{\mur},\ab^{\muc}) = \varphi(\ab^{\mur})-\varphi(\ab^{\muc}) - \langle \nabla\varphi(\ab^{\muc}), \ab^{\mur}-\ab^{\muc} \rangle, \quad \forall (\ab^{\mur},\ab^{\muc}) \in\Omega.
\end{align}
By choosing $\varphi$ appropriately, we can recover several known distances or divergences:
\begin{align}
    \varphi(\x)=\frac{1}{2}\|\x\|^2 &\implies \Delta_{\varphi}(\ab^{\mur},\ab^{\muc})=\|\ab^{\mur}-\ab^{\muc}\|^2\\
    \varphi(\x)=\sum_{i=1}^n x_i\log{x_i} &\implies \Delta_{\varphi}(\ab^{\mur},\ab^{\muc}) = \mathrm{KL}\infdivx{\mur}{\muc}\label{eq:KL}\\
    \varphi(\x)=\frac{1}{2}\|\x\|^2_p &\implies \Delta_{\varphi}(\ab^{\mur},\ab^{\muc})=\frac{1}{2}\|\ab^{\mur}\|^2_p + \frac{1}{2}\|\ab^{\muc}\|^2_p - \langle \nabla \frac{1}{2}\|\ab^{\muc}\|^2_p, \ab^{\mur} \rangle\nonumber
\end{align}
In general, the Bregman divergence is not a metric, because it is not symmetric (\eg, KL-divergence), and does not satisfy the triangle inequality. 
\end{dfn}

%  :
% By making a simplistic assumption, we use same norm on unbalanced or unnormalized measures.

\begin{dfn}[Generalized KL-divergence]
\label{dfn:GKL}
While KL-divergence can be computed via~\cref{dfn:bregman} as in~\cref{eq:KL}, a generalized version that can work with unbalanced distributions can be worked as in~\cite{miller2023simulation}:
\begin{align}
    \label{eq:GKL}
    \mathrm{GKL}\infdivx{\mur}{\muc}  = \sum\limits_{i=1}^n \left(-\log\left(\frac{a^{\muc}_i}{a^{\mur}_i}\right) + \left(\frac{a^{\muc}_i}{a^{\mur}_i}\right) -1\right){a^{\mur}_i}
\end{align}
\end{dfn}

\begin{dfn}[1-Wasserstein (EM) Distance]
\label{dfn:WS}
For discrete probability measures the TV-norm reduces to $L_1$-norm~\cite{levin2017markov}. With the further assumption that the supports of two distributions are identical and aligned, the $1-$Wasserstein distance can be equivalent to the $L_1$-distance, because the "cost" of moving mass directly corresponds to the absolute difference in mass at each point.
\end{dfn}

\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
}


We describe the methodology in this section. In our approach, we assume that the CAD model is available for training. Initially, we train the SurfEmb pipeline with the CAD model and the images to learn correspondence distributions/ surface features on the object CAD model. We employ the learned surface features to train our rotation distribution estimation pipeline. We employ a similar network to IPDF with an image encoder to map the image to a global feature. The global feature and positionally encoded rotation matrix are passed through an MLP to predict the score for a specific rotation. The same global feature can be concatenated with any random rotation matrix to estimate the unnormalized probability for a specific rotation.  We use the learned surface features on the CAD model to employ a scoring mechanism for rotations for a given image.   

% We employ the SurfEmb CNN to predict the corresponding feature image. Using the 2D features, we estimate the closest 3D correspondence in feature space. We use the 2D coordinate and the corresponding 3D point to learn pose distribution. We sample many pairs of 2D points and their corresponding 3D features. The global feature and the positional encoded rotation matrix are passed through an MLP to predict the score for a score matrix. 
% IPDF employs a contrastive learning-based approach where the ground truth rotation is maximized and other random rotations are minimized. IPDF needs an exhaustive sampling of viewpoints to learn the pose distribution of the entire SO3 space.


1.    
